AToM: Amortized Text-to-Mesh using 2D Diffusion

We introduce Amortized Text-to-Mesh (AToM), a feed-forward text-to-mesh framework optimized across multiple text prompts simultaneously. In contrast to existing text-to-3D methods that often entail time-consuming per-prompt optimization and commonly output representations other than polygonal meshes, AToM directly generates high-quality textured meshes in less than 1 second with around 10 times reduction in the training cost, and generalizes to unseen prompts. Our key idea is a novel triplane-based text-to-mesh architecture with a two-stage amortized optimization strategy that ensures stable training and enables scalability. Through extensive experiments on various prompt benchmarks, AToM significantly outperforms state-of-the-art amortized approaches with over 4 times higher accuracy (in DF415 dataset) and produces more distinguishable and higher-quality 3D outputs. AToM demonstrates strong generalizability, offering finegrained 3D assets for unseen interpolated prompts without further optimization during inference, unlike per-prompt solutions.

==> figures/df10_freq.tex <==
\begin{figure*}[h]
\centering
\includegraphics[width=1.0\textwidth]{figures/src/df10k/df10k_freq.png}
\caption{\textbf{Word frequency of DF10K.} DF10K has an unbalanced frequency of each world, making it a challenging benchmark.}
\label{fig:df10k_freq}
\end{figure*}


==> figures/df10k-2.tex <==
\begin{figure*}[h]
\centering
\includegraphics[width=1.0\textwidth]{figures/src/df10k/df10k-6.jpg}
\caption{AToM evaluated in another 440 random prompts from DF10K. See Line2643-3083 in ``prompts/df10k.json'' for text prompts.}
\label{fig:df10k-2}
\end{figure*}


==> figures/df10k.tex <==
\begin{figure*}[h]
\centering
\includegraphics[width=1.0\textwidth]{figures/src/df10k/df10k-1.jpg}
\caption{AToM evaluated in DF10K. AToM handles large-scale dataset while ATT3D suffers from divergent optimization. See Line443-883 in ``prompts/df10k.json'' for text prompts.}
\label{fig:df10k}
\end{figure*}


==> figures/df415.tex <==
\begin{figure*}[h]
\centering
\includegraphics[width=1.0\textwidth]{figures/src/df415/df415.jpg}
\caption{\textbf{Gallery of AToM evaluated in DF415.}}
\label{fig:df415}
\end{figure*}


==> figures/unseen.tex <==
\begin{figure*}[t]
\centering
\includegraphics{example-image-a}
\caption{\textbf{Unseen Prompts} }
\label{fig:visual}
\end{figure*}


==> sections/intro_legal.tex <==
\section{Introduction}
\label{sec:intro}

Polygonal meshes constitute a widely used and efficient representation of 3D shapes. As we step into a revolutionary phase of Generative AI \cite{DiffusionModels, LDM}, the creation of 3D meshes has become increasingly intuitive, with controls transitioning from complex, handcrafted graphics handles to simple textual inputs \cite{Text2mesh, DreamFields, DreamFusion}. However, the majority of text-to-mesh (ToM) techniques \cite{Magic3D, Fantasia3D,TextMesh} require per-prompt optimization process that typically consumes more than one GPU hour. Such expensive training limits their applicability and scalability.


ATT3D \cite{ATT3D} attempts to accelerate text-to-3D generation by amortized optimization \cite{amortizedop}, which trains one unified text-to-3D model on all prompts simultaneously. 3D object for each prompt can then be generated by a simple feed-forward pass without further optimization during inference \cite{ATT3D}. However, the efficacy of ATT3D and most text-to-3D models \cite{DreamFusion, SJC, Latent-NeRF, Shap-E, SDFusion}, is limited predominantly to 3D objects represented by Neural Radiance Fields (NeRF) \cite{NeRF}. 
Converting NeRFs to meshes is inaccurate and costly,  
hence, getting high-quality, high-resolution meshes within seconds is infeasible for the current text-to-3D methods. 


In this work, we aim to generate high-quality textured meshes from texts efficiently. 
\textit{We observe that a simple extension of ATT3D to mesh generation suffers from unstable training and poor geometry.} We find that the \textbf{instability} mainly stems from two primary facets: the \textbf{text-to-mesh architecture} and the \textbf{network optimization}.
First, HyperNetwork \cite{HyperNetworks} for text-to-NeRF generation used in ATT3D introduces numerical instability and demands special layers such as spectral normalization \cite{SpectralNorm}. Extending ATT3D to direct mesh generation suffers even more from this architecture instability, leading to divergent optimization. 
Second, a trivial end-to-end training for text-to-mesh also raises instability due to the topology constraints of the differential mesh representation, \eg DMTet\cite{DMTet}, resulting in poor geometry generation.


We thus introduce \textit{AToM}, the first \textit{a}mortized approach for direct \textit{T}ext-to-\textit{M}esh generation. 
To address architecture instability, AToM introduces a \textit{text-to-triplane} network in replacement of HyperNet for the positional encoding. Text-to-triplane is much more robust to changes in parameters and produces a higher quality of generated 3D content in most cases compared to the HyperNet counterpart. 
The triplane features are used as input to subsequent separated SDF, deformation, and color networks to generate the geometry and texture information for the DMTet mesh representation.
Instead of end-to-end training, we propose a two-stage optimization mechanism. 
The first stage of AToM trains text-to-triplane, SDF, and color networks through low-resolution ( $64\times64$) volumetric rendering guided by a diffusion prior. 
Due to the fact that volumetric rendering takes many points into consideration per ray, it leads to stable optimization for the SDF network. 
The second stage of AToM refines these networks and learns additional deformation networks to shift the mesh vertices. Thanks to the efficient rasterization of the mesh, $1024\times1024$ resolution renderings can thus be applied for the second stage. After the model is trained, AToM can be inferenced by the last stage and generate a high-resolution textured mesh in a few seconds. 


% We train AToM in all prompts simultaneously in each benchmark including the ones used in ATT3D, Pig64, DF27, DF400, and our DF10K generated by a large language model \cite{ChatGPT}. We show AToM achieves close performance to the per-prompt text-to-mesh techniques \cite{Magic3D, Fantasia3D} with over $10\times$ reduction in the optimization cost and being more robust to training parameters. AToM also outperforms ATT3D by a large margin quantitatively and qualitatively. 


\noindent \textbf{Contributions} are listed as follows:
\begin{itemize}[leftmargin=10pt,nosep]
\item We propose AToM, the first amortized text-to-mesh framework. AToM trains a 3D-aware text-to-triplane network, an SDF network, a deformation network, and a color network on all prompts simultaneously. 
We show that our triplane network and separate geometry and texture modeling lead to more stable training and higher quality generation compared to the architecture of ATT3D \cite{ATT3D}. 
\item We introduce a two-stage training, where the first stage uses low-resolution volumetric rendering, and the second stage utilizes high-resolution mesh rasterization. Our two-stage amortized training significantly improves the quality of the texture mesh. 
\item AToM reduces training time by more than $10\times$ compared to per-prompt optimization based solutions such as DreamFusion \cite{DreamFusion} and Fantasia3D \cite{Fantasia3D}. AToM generates high-quality textured meshes in less than 2 seconds, with no post processing required.  AToM also shows strong generalizability to unseen prompts.  

\end{itemize}
\input{figures/pipeline}

==> tables/ablation.tex <==
\begin{table*}[h]
\centering
\vspace{-1em}
\caption{\textbf{Quantitative ablation study} in DF415.
Single stage in column 2 denotes training AToM end-to-end without warm up. 
First stage in column 3 and  other columns at the right show results of first-stage optimization. 
Triplane$\rightarrow$Hyper-INGP in column 4 indicates replacing text-to-triplane with HyperNetworks-based positional encoding used in ATT3D. Column 5 without ConvNeXt indicates using two linear layers with hidden size 32 and spectral normalization for text-to-triplane following Hyper-INGP. 
}
\label{table:ablation}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccccccc}
\textbf{AToM} (Full) 
& single stage
& first stage & triplane$\rightarrow$Hyper-INGP & w/o ConvNeXt
& w/o 3D-aware conv  & w/o cross attention
% & AToM per-prompt
\\
\midrule
 0.8193 & 0.0747 & 0.8169 & 0.3518 & 0.7711 & 0.7976 & 0.7928
\end{tabular}
}
\end{table*}


==> tables/amortized.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Compare AToM to ATT3D} on DF415 and our DF10K. Average CLIP-Similarity$\uparrow$ / CLIP R-probability$\uparrow$ are reported.}
\label{table:sota}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}l|lcccccccc}
\textbf{Dataset}
& ATT3D \cite{ATT3D} & ATT3D-IF$^{*}$ & \textbf{AToM} (\textbf{Ours})\\
\midrule
DF415  \\ 
DF10K 
\end{tabular}
}
\end{table}


==> tables/pig.tex <==
\begin{table*}[t]
\centering
\caption{\textbf{Compare AToM to the state-of-the-art} text-to-3D. CLIP R-probability$\uparrow$ is reported. The per-prompt methods in seen prompts are \demph{deemphasized}. ATT3D-IF$^{*}$ denotes our reproduced ATT3D \cite{ATT3D} using Deep Floyd \cite{DeepFloyd} as diffusion prior. \textbf{Bold} reflects the best.}
\label{table:pig}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}l|cccccccc}
\textbf{Dataset}
% & Point-E \cite{Point-E}
% & Shap-E \cite{Shap-E}
& DreamFusion-IF \cite{DreamFusion, threestudio}  & TextMesh-IF \cite{TextMesh, threestudio} & Fantasia3D \cite{Fantasia3D, threestudio}  & Magic3D-IF \cite{Magic3D, threestudio} &ATT3D \cite{ATT3D} & ATT3D-IF$^{*}$ & \textbf{AToM} (\textbf{Ours})\\
\midrule
\textbf{Pig64 unseen} & 0.1250 & 0.1250 & 0.1250 & 0.1250 & 0.3750 & 0.6250 & \textbf{0.7500} \\
\textbf{Pig64 seen} & \demph{0.7143} & \demph{0.8036} & \demph{0.5357} & \demph{0.8036}& 0.6071 & 0.6250 & 0.7500   \\
\textbf{Pig64 all} &  0.6406 & 0.7188 & 0.4843 & 0.7188 & 0.5781 & 0.6250 & \textbf{0.7500} \\ 
\end{tabular}
}
\end{table*}


